S-polarized light-sheets improve resolution and light-efficiency in oblique plane microscopy

Oblique plane microscopy (OPM) offers 3D optically sectioned imaging with high spatial- and temporal-resolution while enabling conventional sample mounting. The technique uses a concatenation of three microscopes, two for remote focusing and a tilted tertiary microscope, often including an immersion objective, to image an oblique sample plane. This design induces Fresnel reflections and a reduced effective aperture, thus impacting the resolution and light efficiency of the system. Using vectorial diffraction simulations, the system performance was characterized based on illumination angle and polarization, signal to noise ratio, and refractive index of the tertiary objective immersion. We show that for samples with high fluorescent anisotropy, s-polarized light-sheets yield higher average resolution for all system configurations, as well as higher light-efficiency. We also provide a tool for performance characterization of arbitrary light-sheet imaging systems.

==> Supplementary_information/formating.tex <==
\usepackage{authblk} % To use affiliations
\usepackage{graphicx} % Required for inserting images
\usepackage{lineno} % Line numbers
\usepackage{siunitx} % Required for alignment
\usepackage{upgreek} % Required for greek letters in text
\usepackage{cancel} % Required for crossing out text
\usepackage{varwidth} % Required for the text width of cells
\usepackage[utf8]{inputenc} % Required for special characters
\usepackage{amsmath,amsfonts,amssymb,amsthm,mathtools} % Required for some math elements
\usepackage[a4paper, total={7in, 9in}]{geometry}

%Packagaes for figures and tables
\usepackage{graphicx} % Graphics package
\usepackage{subcaption} % To have subfigures
\usepackage{wrapfig} % To wrap text around figures	
\usepackage{float} % To force figures to be placed in the right place

\usepackage{makeidx} % To make an index
\usepackage{color} % To use colors
\usepackage{hyperref} % To use hyperlinks
\usepackage{upgreek}

\usepackage[backend=biber,style=ieee,]{biblatex} % To use bibliography

\usepackage{siunitx}  %Write units easily \SI{value}

% To use code
\usepackage{listings} % To include code
\lstset{
basicstyle=\footnotesize\ttfamily,
identifierstyle=\bfseries\color{green!40!black},
commentstyle=\itshape\color{purple!40!black},
keywordstyle=\color{blue},
stringstyle=\color{orange}} % To set the style of the code

\usepackage{pdfpages} % To include pdf files
\usepackage{lscape} % To rotate pages

\usepackage{footnote} % To use footnotes
\usepackage{sidecap} % To use side captions
\usepackage{appendix} % To use appendices

% Table packages
\usepackage{tabularx} % To use tables
\makesavenoteenv{tabular} % To use footnotes in tables
\makesavenoteenv{table} % To use footnotes in tables
\usepackage{array} % To use tables
\usepackage{booktabs} % To use tables
\newcommand*\rot{\rotatebox{90}} % To rotate text in tables

%Special in-document vector graphics:
\usepackage{tikz}
\usetikzlibrary{shapes.geometric,calc,positioning,3d,intersections,arrows}
\usetikzlibrary{decorations.markings}
\usepackage{pgfplots}
\pgfplotsset{compat=1.14}
\usepackage{circuitikz}  %Brukes til å enkelt tegne kretser

\usepackage{titling}
\setlength{\droptitle}{-8ex}
\pretitle{\begin{flushleft}\Large\bfseries}
\posttitle{\par\end{flushleft}}
\preauthor{\begin{flushleft}\Large}
\postauthor{\end{flushleft}}
\predate{\begin{flushleft}}
\postdate{\end{flushleft}}
% \usepackage{lineno}
% \linenumbers


==> setup.tex <==
\usepackage{authblk} % To use affiliations
\usepackage{graphicx} % Required for inserting images
\usepackage{lineno} % Line numbers
\usepackage{siunitx} % Required for alignment
\usepackage{upgreek} % Required for greek letters in text
\usepackage{cancel} % Required for crossing out text
\usepackage{varwidth} % Required for the text width of cells
\usepackage[utf8]{inputenc} % Required for special characters
\usepackage{amsmath,amsfonts,amssymb,amsthm,mathtools} % Required for some math elements
\usepackage[a4paper, total={7in, 9in}]{geometry}

%Packagaes for figures and tables
\usepackage{graphicx} % Graphics package
\usepackage{subcaption} % To have subfigures
\usepackage{wrapfig} % To wrap text around figures	
\usepackage{float} % To force figures to be placed in the right place

\usepackage{makeidx} % To make an index
\usepackage{color} % To use colors
\usepackage{hyperref} % To use hyperlinks

\usepackage[backend=biber,style=ieee,]{biblatex} % To use bibliography

\usepackage{siunitx}  %Write units easily \SI{value}

% To use code
\usepackage{listings} % To include code
\lstset{
basicstyle=\footnotesize\ttfamily,
identifierstyle=\bfseries\color{green!40!black},
commentstyle=\itshape\color{purple!40!black},
keywordstyle=\color{blue},
stringstyle=\color{orange}} % To set the style of the code

\usepackage{pdfpages} % To include pdf files
\usepackage{lscape} % To rotate pages

\usepackage{footnote} % To use footnotes
\usepackage{sidecap} % To use side captions
\usepackage{appendix} % To use appendices

% Table packages
\usepackage{tabularx} % To use tables
\makesavenoteenv{tabular} % To use footnotes in tables
\makesavenoteenv{table} % To use footnotes in tables
\usepackage{array} % To use tables
\usepackage{booktabs} % To use tables
\newcommand*\rot{\rotatebox{90}} % To rotate text in tables

%Special in-document vector graphics:
\usepackage{tikz}
\usetikzlibrary{shapes.geometric,calc,positioning,3d,intersections,arrows}
\usetikzlibrary{decorations.markings}
\usepackage{pgfplots}
\pgfplotsset{compat=1.14}
\usepackage{circuitikz}  %Brukes til å enkelt tegne kretser

\usepackage{titling}
\setlength{\droptitle}{-8ex}
\pretitle{\begin{flushleft}\Large\bfseries}
\posttitle{\par\end{flushleft}}
\preauthor{\begin{flushleft}\Large}
\postauthor{\end{flushleft}}
\predate{\begin{flushleft}}
\postdate{\end{flushleft}}
